Automated Selfish Mining Analysis for DAG-Based PoW Consensus Protocols

Selfish mining is strategic rule-breaking to maximize rewards in proof-of-work protocols. Markov Decision Processes (MDPs) are the preferred tool for finding optimal strategies in Bitcoin and similar linear chain protocols. Protocols increasingly adopt DAG-based chain structures, for which MDP analysis is more involved. To date, researchers have tailored specific MDPs for each protocol. Protocol design suffers long feedback loops, as each protocol change implies manual work on the MDP. To overcome this, we propose a generic attack model that covers a wide range of protocols, including Ethereum Proof-of-Work, GhostDAG, and Parallel Proof-of-Work. Our approach is modular: we specify each protocol as a concise program, and our tooling then derives and solves the selfish mining MDP automatically.

==> listings/bitcoin.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{k}{def} \PY{n+nf}{init}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{state}\PY{o}{.}\PY{n}{head} \PY{o}{=} \PY{n}{genesis}

\PY{k}{def} \PY{n+nf}{mining}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{p}{\PYZob{}}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{\PYZcb{}}

\PY{k}{def} \PY{n+nf}{update}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{if} \PY{n}{height}\PY{p}{(}\PY{n}{block}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{n}{height}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}\PY{p}{:}
        \PY{n}{state}\PY{o}{.}\PY{n}{head} \PY{o}{=} \PY{n}{block}

\PY{k}{def} \PY{n+nf}{history}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{def} \PY{n+nf}{history\PYZus{}of}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
        \PY{k}{if} \PY{n}{block} \PY{o}{==} \PY{n}{genesis}\PY{p}{:}
            \PY{k}{return} \PY{p}{[}\PY{n}{genesis}\PY{p}{]}
        \PY{k}{else}\PY{p}{:}
            \PY{k}{return} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{parents}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{o}{.}\PY{n}{pop}\PY{p}{(}\PY{p}{)}\PY{p}{)} \PY{o}{+} \PY{p}{[}\PY{n}{block}\PY{p}{]}

    \PY{k}{return} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{progress}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{l+m+mi}{1}

\PY{k}{def} \PY{n+nf}{coinbase}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{p}{[}\PY{p}{(}\PY{n}{miner\PYZus{}of}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{,} \PY{l+m+mi}{1}\PY{p}{)}\PY{p}{]}
\end{Verbatim}


==> listings/byzantium.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{k}{def} \PY{n+nf}{mining}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{uncles} \PY{o}{=} \PY{n}{available\PYZus{}uncles}\PY{p}{(}\PY{p}{)}
    \PY{c+c1}{\PYZsh{} choose at most 2 uncles, own blocks first}
    \PY{n}{ranked} \PY{o}{=} \PY{n+nb}{sorted}\PY{p}{(}\PY{n}{uncles}\PY{p}{,} \PY{n}{key}\PY{o}{=}\PY{k}{lambda} \PY{n}{u}\PY{p}{:} \PY{n}{miner\PYZus{}of}\PY{p}{(}\PY{n}{u}\PY{p}{)} \PY{o}{!=} \PY{n}{me}\PY{p}{)}
    \PY{k}{return} \PY{p}{\PYZob{}}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{\PYZcb{}} \PY{o}{|} \PY{n+nb}{set}\PY{p}{(}\PY{n}{ranked}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{:}\PY{l+m+mi}{2}\PY{p}{]}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{update}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{n}{prg\PYZus{}new} \PY{o}{=} \PY{n+nb}{sum}\PY{p}{(}\PY{n}{progress}\PY{p}{(}\PY{n}{b}\PY{p}{)} \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{)}
    \PY{n}{prg\PYZus{}old} \PY{o}{=} \PY{n+nb}{sum}\PY{p}{(}\PY{n}{progress}\PY{p}{(}\PY{n}{b}\PY{p}{)} \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}\PY{p}{)}
    \PY{k}{if} \PY{n}{prg\PYZus{}new} \PY{o}{\PYZgt{}} \PY{n}{prg\PYZus{}old}\PY{p}{:}
        \PY{n}{state}\PY{o}{.}\PY{n}{head} \PY{o}{=} \PY{n}{block}

\PY{k}{def} \PY{n+nf}{progress}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{n}{\PYZus{}}\PY{p}{,} \PY{n}{uncles} \PY{o}{=} \PY{n}{parent\PYZus{}and\PYZus{}uncles}\PY{p}{(}\PY{n}{block}\PY{p}{)}
    \PY{k}{return} \PY{l+m+mi}{1} \PY{o}{+} \PY{n+nb}{len}\PY{p}{(}\PY{n}{uncles}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{coinbase}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{n}{\PYZus{}}\PY{p}{,} \PY{n}{uncles} \PY{o}{=} \PY{n}{parent\PYZus{}and\PYZus{}uncles}\PY{p}{(}\PY{n}{block}\PY{p}{)}
    \PY{n}{lst} \PY{o}{=} \PY{p}{[}\PY{p}{(}\PY{n}{miner\PYZus{}of}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{,} \PY{l+m+mi}{1} \PY{o}{+} \PY{l+m+mf}{0.03125} \PY{o}{*} \PY{n+nb}{len}\PY{p}{(}\PY{n}{uncles}\PY{p}{)}\PY{p}{)}\PY{p}{]}
    \PY{n}{h} \PY{o}{=} \PY{n}{height}\PY{p}{(}\PY{n}{block}\PY{p}{)}
    \PY{n}{max\PYZus{}d} \PY{o}{=} \PY{n}{h} \PY{o}{+} \PY{l+m+mi}{1}
    \PY{k}{for} \PY{n}{u} \PY{o+ow}{in} \PY{n}{uncles}\PY{p}{:}
        \PY{n}{d} \PY{o}{=} \PY{n}{h} \PY{o}{\PYZhy{}} \PY{n}{height}\PY{p}{(}\PY{n}{u}\PY{p}{)}
        \PY{n}{lst}\PY{o}{.}\PY{n}{append}\PY{p}{(}\PY{p}{(}\PY{n}{miner\PYZus{}of}\PY{p}{(}\PY{n}{u}\PY{p}{)}\PY{p}{,} \PY{p}{(}\PY{n}{max\PYZus{}d} \PY{o}{\PYZhy{}} \PY{n}{d}\PY{p}{)} \PY{o}{/} \PY{n}{max\PYZus{}d}\PY{p}{)}\PY{p}{)}
    \PY{k}{return} \PY{n}{lst}
\end{Verbatim}


==> listings/ethereum.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{n}{h}\PY{p}{:} \PY{n+nb}{int} \PY{o}{=} \PY{l+m+mi}{3}

\PY{k}{def} \PY{n+nf}{init}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{state}\PY{o}{.}\PY{n}{head} \PY{o}{=} \PY{n}{genesis}

\PY{k}{def} \PY{n+nf}{mining}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{p}{\PYZob{}}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{\PYZcb{}} \PY{o}{|} \PY{n}{available\PYZus{}uncles}\PY{p}{(}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{available\PYZus{}uncles}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{hist} \PY{o}{=} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}
    \PY{n}{allowed\PYZus{}parents} \PY{o}{=} \PY{n+nb}{set}\PY{p}{(}\PY{n}{hist}\PY{p}{[}\PY{o}{\PYZhy{}}\PY{n}{h} \PY{o}{\PYZhy{}} \PY{l+m+mi}{1} \PY{p}{:} \PY{o}{\PYZhy{}}\PY{l+m+mi}{2}\PY{p}{]}\PY{p}{)}
    \PY{n}{uncles} \PY{o}{=} \PY{n+nb}{set}\PY{p}{(}\PY{p}{)}
    \PY{n}{leaves} \PY{o}{=} \PY{p}{\PYZob{}}\PY{n}{b} \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{n}{G} \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{children}\PY{p}{(}\PY{n}{b}\PY{p}{)}\PY{p}{)} \PY{o}{==} \PY{l+m+mi}{0}\PY{p}{\PYZcb{}}
    \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{n}{leaves}\PY{p}{:}
        \PY{n}{p}\PY{p}{,} \PY{n}{\PYZus{}} \PY{o}{=} \PY{n}{parent\PYZus{}and\PYZus{}uncles}\PY{p}{(}\PY{n}{b}\PY{p}{)}
        \PY{k}{if} \PY{n}{p} \PY{o+ow}{in} \PY{n}{allowed\PYZus{}parents}\PY{p}{:}
            \PY{n}{uncles}\PY{o}{.}\PY{n}{add}\PY{p}{(}\PY{n}{b}\PY{p}{)}
    \PY{k}{return} \PY{n}{uncles}

\PY{k}{def} \PY{n+nf}{update}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{if} \PY{n}{height}\PY{p}{(}\PY{n}{block}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{n}{height}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}\PY{p}{:}
        \PY{n}{state}\PY{o}{.}\PY{n}{head} \PY{o}{=} \PY{n}{block}

\PY{k}{def} \PY{n+nf}{history\PYZus{}of}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{if} \PY{n}{block} \PY{o}{==} \PY{n}{genesis}\PY{p}{:}
        \PY{k}{return} \PY{p}{[}\PY{n}{genesis}\PY{p}{]}
    \PY{k}{else}\PY{p}{:}
        \PY{n}{parent}\PY{p}{,} \PY{n}{\PYZus{}} \PY{o}{=} \PY{n}{parent\PYZus{}and\PYZus{}uncles}\PY{p}{(}\PY{n}{block}\PY{p}{)}
        \PY{k}{return} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{parent}\PY{p}{)} \PY{o}{+} \PY{p}{[}\PY{n}{block}\PY{p}{]}

\PY{k}{def} \PY{n+nf}{parent\PYZus{}and\PYZus{}uncles}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{n}{ranked} \PY{o}{=} \PY{n+nb}{sorted}\PY{p}{(}\PY{n}{parents}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{,} \PY{n}{key}\PY{o}{=}\PY{k}{lambda} \PY{n}{p}\PY{p}{:} \PY{o}{\PYZhy{}}\PY{n}{height}\PY{p}{(}\PY{n}{p}\PY{p}{)}\PY{p}{)}
    \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{ranked}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{l+m+mi}{0}\PY{p}{:}
        \PY{k}{return} \PY{n}{ranked}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}\PY{p}{,} \PY{n+nb}{set}\PY{p}{(}\PY{n}{ranked}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{:}\PY{p}{]}\PY{p}{)}
    \PY{k}{else}\PY{p}{:}
        \PY{k}{return} \PY{k+kc}{None}\PY{p}{,} \PY{n+nb}{set}\PY{p}{(}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{history}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{progress}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{l+m+mi}{1}

\PY{k}{def} \PY{n+nf}{coinbase}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{n}{\PYZus{}}\PY{p}{,} \PY{n}{uncles} \PY{o}{=} \PY{n}{parent\PYZus{}and\PYZus{}uncles}\PY{p}{(}\PY{n}{block}\PY{p}{)}
    \PY{k}{return} \PY{p}{[}\PY{p}{(}\PY{n}{miner\PYZus{}of}\PY{p}{(}\PY{n}{b}\PY{p}{)}\PY{p}{,} \PY{l+m+mi}{1}\PY{p}{)} \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{p}{\PYZob{}}\PY{n}{block}\PY{p}{\PYZcb{}} \PY{o}{|} \PY{n}{uncles}\PY{p}{]}
\end{Verbatim}


==> listings/ghostdag.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{n}{k}\PY{p}{:} \PY{n+nb}{int} \PY{o}{=} \PY{l+m+mi}{3}

\PY{k}{def} \PY{n+nf}{mining}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{n}{tips}\PY{p}{(}\PY{n}{G}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{history\PYZus{}of}\PY{p}{(}\PY{n}{G}\PY{p}{)}\PY{p}{:}  \PY{c+c1}{\PYZsh{} eprint.iacr.org/2018/104.pdf ; Alg. 1}
    \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{G}\PY{p}{)} \PY{o}{==} \PY{l+m+mi}{1}\PY{p}{:}
        \PY{k}{return} \PY{p}{(}\PY{p}{\PYZob{}}\PY{n}{genesis}\PY{p}{\PYZcb{}}\PY{p}{,} \PY{p}{[}\PY{n}{genesis}\PY{p}{]}\PY{p}{)}

    \PY{n}{blue}\PY{p}{,} \PY{n}{hist} \PY{o}{=} \PY{n+nb}{dict}\PY{p}{(}\PY{p}{)}\PY{p}{,} \PY{n+nb}{dict}\PY{p}{(}\PY{p}{)}
    \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{n}{tips}\PY{p}{(}\PY{n}{G}\PY{p}{)}\PY{p}{:}
        \PY{n}{blue}\PY{p}{[}\PY{n}{b}\PY{p}{]}\PY{p}{,} \PY{n}{hist}\PY{p}{[}\PY{n}{b}\PY{p}{]} \PY{o}{=} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{past}\PY{p}{(}\PY{n}{G}\PY{p}{,} \PY{n}{b}\PY{p}{)}\PY{p}{)}
    \PY{n}{b\PYZus{}max} \PY{o}{=} \PY{n+nb}{sorted}\PY{p}{(}\PY{n}{tips}\PY{p}{(}\PY{n}{G}\PY{p}{)}\PY{p}{,} \PY{n}{key}\PY{o}{=}\PY{k}{lambda} \PY{n}{b}\PY{p}{:} \PY{p}{(}\PY{o}{\PYZhy{}}\PY{n+nb}{len}\PY{p}{(}\PY{n}{blue}\PY{p}{[}\PY{n}{b}\PY{p}{]}\PY{p}{)}\PY{p}{,} \PY{n+nb}{hash}\PY{p}{(}\PY{n}{b}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{]}
    \PY{n}{blue} \PY{o}{=} \PY{n}{blue}\PY{p}{[}\PY{n}{b\PYZus{}max}\PY{p}{]} \PY{o}{|} \PY{p}{\PYZob{}}\PY{n}{b\PYZus{}max}\PY{p}{\PYZcb{}}
    \PY{n}{hist} \PY{o}{=} \PY{n}{hist}\PY{p}{[}\PY{n}{b\PYZus{}max}\PY{p}{]} \PY{o}{+} \PY{p}{[}\PY{n}{b\PYZus{}max}\PY{p}{]}

    \PY{n}{ac} \PY{o}{=} \PY{n}{anticone}\PY{p}{(}\PY{n}{G}\PY{p}{,} \PY{n}{b\PYZus{}max}\PY{p}{)}
    \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{n+nb}{sorted}\PY{p}{(}\PY{n}{ac}\PY{p}{,} \PY{n}{key}\PY{o}{=}\PY{k}{lambda} \PY{n}{b}\PY{p}{:} \PY{p}{(}\PY{n}{height}\PY{p}{(}\PY{n}{b}\PY{p}{)}\PY{p}{,} \PY{n+nb}{hash}\PY{p}{(}\PY{n}{b}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{:}
        \PY{k}{if} \PY{n}{is\PYZus{}k\PYZus{}cluster}\PY{p}{(}\PY{n}{G}\PY{p}{,} \PY{n}{blue} \PY{o}{|} \PY{p}{\PYZob{}}\PY{n}{b}\PY{p}{\PYZcb{}}\PY{p}{)}\PY{p}{:}
            \PY{n}{blue} \PY{o}{=} \PY{n}{blue} \PY{o}{|} \PY{p}{\PYZob{}}\PY{n}{b}\PY{p}{\PYZcb{}}
            \PY{n}{hist} \PY{o}{=} \PY{n}{hist} \PY{o}{+} \PY{p}{[}\PY{n}{b}\PY{p}{]}  \PY{c+c1}{\PYZsh{} only blue blocks get a reward}

    \PY{k}{return} \PY{p}{(}\PY{n}{blue}\PY{p}{,} \PY{n}{hist}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{is\PYZus{}k\PYZus{}cluster}\PY{p}{(}\PY{n}{G}\PY{p}{,} \PY{n}{S}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{n+nb}{all}\PY{p}{(}\PY{n+nb}{len}\PY{p}{(}\PY{n}{anticone}\PY{p}{(}\PY{n}{G}\PY{p}{,} \PY{n}{b}\PY{p}{)} \PY{o}{\PYZam{}} \PY{n}{S}\PY{p}{)} \PY{o}{\PYZlt{}}\PY{o}{=} \PY{n}{k} \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{n}{S}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{history}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{\PYZus{}blue}\PY{p}{,} \PY{n}{history} \PY{o}{=} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{G}\PY{p}{)}
    \PY{k}{return} \PY{n}{history}

\PY{c+c1}{\PYZsh{} init() and fn update() do nothing}
\PY{c+c1}{\PYZsh{} progress() and coinbase() are like in Bitcoin}
\end{Verbatim}


==> listings/ghostdag_util.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{c+c1}{\PYZsh{} protocol helper functions}

\PY{k}{def} \PY{n+nf}{tips}\PY{p}{(}\PY{n}{subgraph}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{p}{\PYZob{}}\PY{n}{b} \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{n}{subgraph} \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{children}\PY{p}{(}\PY{n}{b}\PY{p}{)} \PY{o}{\PYZam{}} \PY{n}{subgraph}\PY{p}{)} \PY{o}{==} \PY{l+m+mi}{0}\PY{p}{\PYZcb{}}

\PY{k}{def} \PY{n+nf}{past\PYZus{}or\PYZus{}future}\PY{p}{(}\PY{n}{relation}\PY{p}{,} \PY{n}{subgraph}\PY{p}{,} \PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{n}{acc} \PY{o}{=} \PY{n+nb}{set}\PY{p}{(}\PY{p}{)}
    \PY{n}{stack} \PY{o}{=} \PY{n+nb}{set}\PY{p}{(}\PY{n}{relation}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{)} \PY{o}{\PYZam{}} \PY{n}{subgraph}
    \PY{k}{while} \PY{n+nb}{len}\PY{p}{(}\PY{n}{stack}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{l+m+mi}{0}\PY{p}{:}
        \PY{n}{b} \PY{o}{=} \PY{n}{stack}\PY{o}{.}\PY{n}{pop}\PY{p}{(}\PY{p}{)}
        \PY{k}{if} \PY{n}{b} \PY{o+ow}{not} \PY{o+ow}{in} \PY{n}{acc}\PY{p}{:}
            \PY{n}{acc}\PY{o}{.}\PY{n}{add}\PY{p}{(}\PY{n}{b}\PY{p}{)}
            \PY{k}{for} \PY{n}{p} \PY{o+ow}{in} \PY{n+nb}{set}\PY{p}{(}\PY{n}{relation}\PY{p}{(}\PY{n}{b}\PY{p}{)}\PY{p}{)} \PY{o}{\PYZam{}} \PY{n}{subgraph}\PY{p}{:}
                \PY{n}{stack}\PY{o}{.}\PY{n}{add}\PY{p}{(}\PY{n}{p}\PY{p}{)}
    \PY{k}{return} \PY{n}{acc}

\PY{k}{def} \PY{n+nf}{past}\PY{p}{(}\PY{n}{subgraph}\PY{p}{,} \PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{n}{past\PYZus{}or\PYZus{}future}\PY{p}{(}\PY{n}{parents}\PY{p}{,} \PY{n}{subgraph}\PY{p}{,} \PY{n}{block}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{future}\PY{p}{(}\PY{n}{subgraph}\PY{p}{,} \PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{n}{past\PYZus{}or\PYZus{}future}\PY{p}{(}\PY{n}{children}\PY{p}{,} \PY{n}{subgraph}\PY{p}{,} \PY{n}{block}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{anticone}\PY{p}{(}\PY{n}{subgraph}\PY{p}{,} \PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{p}{(}
        \PY{n}{subgraph}
        \PY{o}{\PYZhy{}} \PY{p}{\PYZob{}}\PY{n}{block}\PY{p}{\PYZcb{}}
        \PY{o}{\PYZhy{}} \PY{n}{past}\PY{p}{(}\PY{n}{subgraph}\PY{p}{,} \PY{n}{block}\PY{p}{)}
        \PY{o}{\PYZhy{}} \PY{n}{future}\PY{p}{(}\PY{n}{subgraph}\PY{p}{,} \PY{n}{block}\PY{p}{)}
    \PY{p}{)}

\PY{c+c1}{\PYZsh{} remaining protocol specification functions}

\PY{k}{def} \PY{n+nf}{init}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{pass}

\PY{k}{def} \PY{n+nf}{update}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{pass}

\PY{k}{def} \PY{n+nf}{progress}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{l+m+mi}{1}

\PY{k}{def} \PY{n+nf}{coinbase}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{p}{[}\PY{p}{(}\PY{n}{miner\PYZus{}of}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{,} \PY{l+m+mi}{1}\PY{p}{)}\PY{p}{]}
\end{Verbatim}


==> listings/parallel.tex <==
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`\$=3\catcode`\^=7\catcode`\_=8\relax}]
\PY{n}{k}\PY{p}{:} \PY{n+nb}{int} \PY{o}{=} \PY{l+m+mi}{3}

\PY{k}{def} \PY{n+nf}{init}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{state}\PY{o}{.}\PY{n}{head} \PY{o}{=} \PY{n}{genesis}

\PY{k}{def} \PY{n+nf}{mining}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{n}{votes} \PY{o}{=} \PY{n}{children}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}
    \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{votes}\PY{p}{)} \PY{o}{\PYZgt{}}\PY{o}{=} \PY{n}{k}\PY{p}{:}
        \PY{c+c1}{\PYZsh{} choose k votes, own votes first}
        \PY{n}{ranked} \PY{o}{=} \PY{n+nb}{sorted}\PY{p}{(}\PY{n}{votes}\PY{p}{,} \PY{n}{key}\PY{o}{=}\PY{k}{lambda} \PY{n}{v}\PY{p}{:} \PY{n}{miner\PYZus{}of}\PY{p}{(}\PY{n}{v}\PY{p}{)} \PY{o}{!=} \PY{n}{me}\PY{p}{)}
        \PY{k}{return} \PY{n+nb}{set}\PY{p}{(}\PY{n}{ranked}\PY{p}{[}\PY{l+m+mi}{0}\PY{p}{:}\PY{n}{k}\PY{p}{]}\PY{p}{)}
    \PY{k}{return} \PY{p}{\PYZob{}}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{\PYZcb{}}

\PY{k}{def} \PY{n+nf}{update}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{if} \PY{n}{is\PYZus{}vote}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
        \PY{n}{block} \PY{o}{=} \PY{n}{parents}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{o}{.}\PY{n}{pop}\PY{p}{(}\PY{p}{)}
    \PY{k}{if} \PY{n}{height}\PY{p}{(}\PY{n}{block}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{n}{height}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}\PY{p}{:}
        \PY{n}{state}\PY{o}{.}\PY{n}{head} \PY{o}{=} \PY{n}{block}
    \PY{k}{elif} \PY{n}{height}\PY{p}{(}\PY{n}{block}\PY{p}{)} \PY{o}{==} \PY{n}{height}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}\PY{p}{:}
        \PY{k}{if} \PY{n+nb}{len}\PY{p}{(}\PY{n}{children}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{n+nb}{len}\PY{p}{(}\PY{n}{children}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}\PY{p}{)}\PY{p}{:}
            \PY{n}{state}\PY{o}{.}\PY{n}{head} \PY{o}{=} \PY{n}{block}

\PY{k}{def} \PY{n+nf}{is\PYZus{}vote}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{n+nb}{len}\PY{p}{(}\PY{n}{parents}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{)} \PY{o}{==} \PY{l+m+mi}{1}

\PY{k}{def} \PY{n+nf}{history\PYZus{}of}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{if} \PY{n}{block} \PY{o}{==} \PY{n}{genesis}\PY{p}{:}
        \PY{k}{return} \PY{p}{[}\PY{n}{genesis}\PY{p}{]}
    \PY{k}{elif} \PY{n}{is\PYZus{}vote}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
        \PY{k}{return} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{parents}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{o}{.}\PY{n}{pop}\PY{p}{(}\PY{p}{)}\PY{p}{)}
    \PY{k}{else}\PY{p}{:}
        \PY{k}{return} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{parents}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{o}{.}\PY{n}{pop}\PY{p}{(}\PY{p}{)}\PY{p}{)} \PY{o}{+} \PY{p}{[}\PY{n}{block}\PY{p}{]}

\PY{k}{def} \PY{n+nf}{history}\PY{p}{(}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{n}{history\PYZus{}of}\PY{p}{(}\PY{n}{state}\PY{o}{.}\PY{n}{head}\PY{p}{)}

\PY{k}{def} \PY{n+nf}{progress}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{n}{k} \PY{o}{+} \PY{l+m+mi}{1}

\PY{k}{def} \PY{n+nf}{coinbase}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{:}
    \PY{k}{return} \PY{p}{[}\PY{p}{(}\PY{n}{miner\PYZus{}of}\PY{p}{(}\PY{n}{b}\PY{p}{)}\PY{p}{,} \PY{l+m+mi}{1}\PY{p}{)} \PY{k}{for} \PY{n}{b} \PY{o+ow}{in} \PY{p}{\PYZob{}}\PY{n}{block}\PY{p}{\PYZcb{}} \PY{o}{|} \PY{n}{parents}\PY{p}{(}\PY{n}{block}\PY{p}{)}\PY{p}{]}
\end{Verbatim}


==> listings/style.tex <==
%
%
%

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\@namedef{PY@tok@w}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\@namedef{PY@tok@c}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cp}{\def\PY@tc##1{\textcolor[rgb]{0.61,0.40,0.00}{##1}}}
\@namedef{PY@tok@k}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kp}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kt}{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\@namedef{PY@tok@o}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@ow}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PY@tok@nb}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@nf}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@nc}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@nn}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@ne}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.80,0.25,0.22}{##1}}}
\@namedef{PY@tok@nv}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@no}{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\@namedef{PY@tok@nl}{\def\PY@tc##1{\textcolor[rgb]{0.46,0.46,0.00}{##1}}}
\@namedef{PY@tok@ni}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PY@tok@na}{\def\PY@tc##1{\textcolor[rgb]{0.41,0.47,0.13}{##1}}}
\@namedef{PY@tok@nt}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@nd}{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PY@tok@s}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sd}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@si}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PY@tok@se}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.36,0.12}{##1}}}
\@namedef{PY@tok@sr}{\def\PY@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PY@tok@ss}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@sx}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@m}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@gh}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PY@tok@gu}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\@namedef{PY@tok@gd}{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\@namedef{PY@tok@gi}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.52,0.00}{##1}}}
\@namedef{PY@tok@gr}{\def\PY@tc##1{\textcolor[rgb]{0.89,0.00,0.00}{##1}}}
\@namedef{PY@tok@ge}{\let\PY@it=\textit}
\@namedef{PY@tok@gs}{\let\PY@bf=\textbf}
\@namedef{PY@tok@gp}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PY@tok@go}{\def\PY@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PY@tok@gt}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\@namedef{PY@tok@err}{\def\PY@bc##1{{\setlength{\fboxsep}{\string -\fboxrule}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}}
\@namedef{PY@tok@kc}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kd}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kn}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@kr}{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@bp}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PY@tok@fm}{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PY@tok@vc}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vg}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vi}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@vm}{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PY@tok@sa}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sb}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sc}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@dl}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@s2}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@sh}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@s1}{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PY@tok@mb}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mf}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mh}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mi}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@il}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@mo}{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PY@tok@ch}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cm}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cpf}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@c1}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PY@tok@cs}{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
%
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother


